Composable Generative Models

Generative modeling has recently seen many exciting developments with the advent of deep generative architectures such as Variational Auto-Encoders (VAE) or Generative Adversarial Networks (GAN). The ability to draw synthetic i.i.d. observations with the same joint probability distribution as a given dataset has a wide range of applications including representation learning, compression or imputation. It appears that it also has many applications in privacy preserving data analysis, especially when used in conjunction with differential privacy techniques. This paper focuses on synthetic data generation models with privacy preserving applications in mind. It introduces a novel architecture, the Composable Generative Model (CGM) that is state-of-the-art in tabular data generation. Any conditional generative model can be used as a sub-component of the CGM, including CGMs themselves, allowing the generation of numerical, categorical data as well as images, text, or time series. The CGM has been evaluated on 13 datasets (6 standard datasets and 7 simulated) and compared to 14 recent generative models. It beats the state of the art in tabular data generation by a significant margin.

==> tables/adult.tex <==
\begin{tabular}{lrr}
\toprule
{} &  adult/accuracy &  adult/f1 \\
\midrule
IndependentSynthesizer         &            0.64 &      0.15 \\
VEEGANSynthesizer              &            0.72 &      0.16 \\
GaussianCopulaOneHot           &            0.78 &      0.20 \\
UniformSynthesizer             &            0.49 &      0.24 \\
MedganSynthesizer              &            0.62 &      0.24 \\
GaussianCopulaCategoricalFuzzy &            0.77 &      0.26 \\
CLBNSynthesizer                &            0.77 &      0.31 \\
TableganSynthesizer            &            0.79 &      0.35 \\
PrivBNSynthesizer              &            0.80 &      0.43 \\
CTGANSynthesizer               &            0.80 &      0.60 \\
CopulaGAN                      &            0.79 &      0.61 \\
CTGAN                          &            0.79 &      0.61 \\
TVAESynthesizer                &            0.80 &      0.62 \\
\textbf{\model (ours)}                 &            0.83 &      0.65 \\
IdentitySynthesizer            &            0.82 &      0.66 \\
\bottomrule
\end{tabular}


==> tables/alarm.tex <==
\begin{tabular}{lrr}
\toprule
{} &  alarm/syn\_likelihood &  alarm/test\_likelihood \\
\midrule
UniformSynthesizer             &                -18.42 &                 -18.42 \\
VEEGANSynthesizer              &                -18.39 &                 -18.21 \\
IndependentSynthesizer         &                -18.24 &                 -15.82 \\
GaussianCopulaOneHot           &                -15.48 &                 -15.67 \\
GaussianCopulaCategorical      &                -12.91 &                 -15.57 \\
GaussianCopulaCategoricalFuzzy &                -14.52 &                 -14.57 \\
MedganSynthesizer              &                 -7.84 &                 -13.26 \\
CTGAN                          &                -15.88 &                 -13.10 \\
CopulaGAN                      &                -15.69 &                 -13.05 \\
CTGANSynthesizer               &                -15.22 &                 -12.93 \\
TableganSynthesizer            &                -12.69 &                 -11.54 \\
CLBNSynthesizer                &                -12.46 &                 -11.19 \\
PrivBNSynthesizer              &                -12.15 &                 -11.14 \\
TVAESynthesizer                &                -11.44 &                 -10.76 \\
\textbf{\model (ours)}                 &                -10.63 &                 -10.48 \\
IdentitySynthesizer            &                -10.23 &                 -10.30 \\
\bottomrule
\end{tabular}


==> tables/asia.tex <==
\begin{tabular}{lrr}
\toprule
{} &  asia/syn\_likelihood &  asia/test\_likelihood \\
\midrule
MedganSynthesizer              &                -1.57 &                 -5.97 \\
VEEGANSynthesizer              &               -11.49 &                 -5.95 \\
UniformSynthesizer             &               -14.28 &                 -5.52 \\
GaussianCopulaCategorical      &                -2.25 &                 -3.61 \\
GaussianCopulaOneHot           &                -2.31 &                 -3.23 \\
GaussianCopulaCategoricalFuzzy &                -2.83 &                 -3.11 \\
IndependentSynthesizer         &                -4.97 &                 -2.99 \\
TableganSynthesizer            &                -3.40 &                 -2.72 \\
CTGAN                          &                -4.19 &                 -2.46 \\
CopulaGAN                      &                -3.96 &                 -2.40 \\
CTGANSynthesizer               &                -2.69 &                 -2.31 \\
CLBNSynthesizer                &                -2.40 &                 -2.27 \\
TVAESynthesizer                &                -2.29 &                 -2.27 \\
\textbf{\model (ours)}                 &                -2.33 &                 -2.25 \\
PrivBNSynthesizer              &                -2.29 &                 -2.24 \\
IdentitySynthesizer            &                -2.24 &                 -2.24 \\
\bottomrule
\end{tabular}


==> tables/census.tex <==
\begin{tabular}{lrr}
\toprule
{} &  census/accuracy &  census/f1 \\
\midrule
GaussianCopulaCategorical      &             0.94 &       0.00 \\
VEEGANSynthesizer              &             0.76 &       0.05 \\
GaussianCopulaCategoricalFuzzy &             0.79 &       0.05 \\
IndependentSynthesizer         &             0.66 &       0.06 \\
UniformSynthesizer             &             0.54 &       0.11 \\
GaussianCopulaOneHot           &             0.93 &       0.13 \\
MedganSynthesizer              &             0.64 &       0.14 \\
PrivBNSynthesizer              &             0.90 &       0.24 \\
TableganSynthesizer            &             0.94 &       0.27 \\
CLBNSynthesizer                &             0.90 &       0.29 \\
CTGAN                          &             0.92 &       0.33 \\
CTGANSynthesizer               &             0.90 &       0.38 \\
TVAESynthesizer                &             0.93 &       0.38 \\
CopulaGAN                      &             0.89 &       0.39 \\
\textbf{\model (ours)}                 &             0.91 &       0.41 \\
IdentitySynthesizer            &             0.91 &       0.46 \\
\bottomrule
\end{tabular}


==> tables/child.tex <==
\begin{tabular}{lrr}
\toprule
{} &  child/syn\_likelihood &  child/test\_likelihood \\
\midrule
UniformSynthesizer             &                -18.41 &                 -18.32 \\
VEEGANSynthesizer              &                -17.31 &                 -17.68 \\
IndependentSynthesizer         &                -17.96 &                 -16.03 \\
GaussianCopulaCategorical      &                -16.40 &                 -15.55 \\
GaussianCopulaCategoricalFuzzy &                -16.90 &                 -15.41 \\
GaussianCopulaOneHot           &                -14.48 &                 -15.31 \\
TableganSynthesizer            &                -15.02 &                 -13.39 \\
MedganSynthesizer              &                -11.11 &                 -12.99 \\
CopulaGAN                      &                -14.25 &                 -12.92 \\
CTGAN                          &                -14.35 &                 -12.84 \\
CTGANSynthesizer               &                -13.81 &                 -12.81 \\
CLBNSynthesizer                &                -12.63 &                 -12.31 \\
TVAESynthesizer                &                -12.46 &                 -12.30 \\
PrivBNSynthesizer              &                -12.36 &                 -12.19 \\
\textbf{\model (ours)}                 &                -11.83 &                 -12.13 \\
IdentitySynthesizer            &                -12.03 &                 -12.04 \\
\bottomrule
\end{tabular}


==> tables/covtype.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  covtype/accuracy &  covtype/macro\_f1 &  covtype/micro\_f1 \\
\midrule
TableganSynthesizer            &              0.00 &              0.00 &              0.00 \\
UniformSynthesizer             &              0.14 &              0.09 &              0.14 \\
VEEGANSynthesizer              &              0.22 &              0.10 &              0.22 \\
IndependentSynthesizer         &              0.38 &              0.11 &              0.38 \\
GaussianCopulaCategoricalFuzzy &              0.42 &              0.14 &              0.42 \\
GaussianCopulaCategorical      &              0.42 &              0.14 &              0.42 \\
MedganSynthesizer              &              0.44 &              0.09 &              0.44 \\
PrivBNSynthesizer              &              0.47 &              0.21 &              0.47 \\
GaussianCopulaOneHot           &              0.51 &              0.18 &              0.51 \\
CLBNSynthesizer                &              0.56 &              0.33 &              0.56 \\
CTGAN                          &              0.57 &              0.32 &              0.57 \\
CopulaGAN                      &              0.57 &              0.33 &              0.57 \\
CTGANSynthesizer               &              0.58 &              0.33 &              0.58 \\
TVAESynthesizer                &              0.65 &              0.46 &              0.65 \\
\textbf{\model (ours)}                 &              0.70 &              0.49 &              0.70 \\
IdentitySynthesizer            &              0.76 &              0.65 &              0.76 \\
\bottomrule
\end{tabular}


==> tables/credit.tex <==
\begin{tabular}{lrr}
\toprule
{} &  credit/accuracy &  credit/f1 \\
\midrule
GaussianCopulaCategorical      &             1.00 &       0.00 \\
GaussianCopulaOneHot           &             1.00 &       0.00 \\
TVAESynthesizer                &             1.00 &       0.00 \\
IndependentSynthesizer         &             0.88 &       0.00 \\
GaussianCopulaCategoricalFuzzy &             0.98 &       0.01 \\
PrivBNSynthesizer              &             0.96 &       0.01 \\
UniformSynthesizer             &             0.57 &       0.01 \\
MedganSynthesizer              &             0.94 &       0.02 \\
VEEGANSynthesizer              &             0.88 &       0.17 \\
TableganSynthesizer            &             1.00 &       0.27 \\
CLBNSynthesizer                &             1.00 &       0.44 \\
CTGANSynthesizer               &             0.99 &       0.52 \\
\textbf{\model (ours)}                 &             1.00 &       0.53 \\
IdentitySynthesizer            &             0.99 &       0.55 \\
CTGAN                          &             1.00 &       0.66 \\
CopulaGAN                      &             1.00 &       0.72 \\
\bottomrule
\end{tabular}


==> tables/grid.tex <==
\begin{tabular}{lrr}
\toprule
{} &  grid/syn\_likelihood &  grid/test\_likelihood \\
\midrule
VEEGANSynthesizer              &                -8.65 &               -423.57 \\
MedganSynthesizer              &                -5.83 &                -90.34 \\
CLBNSynthesizer                &                -3.88 &                 -9.20 \\
PrivBNSynthesizer              &                -3.99 &                 -8.31 \\
TVAESynthesizer                &                -3.27 &                 -5.66 \\
TableganSynthesizer            &                -6.99 &                 -5.33 \\
CopulaGAN                      &                -8.19 &                 -5.14 \\
CTGANSynthesizer               &                -8.92 &                 -5.09 \\
CTGAN                          &                -8.76 &                 -5.06 \\
GaussianCopulaCategoricalFuzzy &                -7.34 &                 -4.57 \\
UniformSynthesizer             &                -7.33 &                 -4.54 \\
GaussianCopulaOneHot           &                -7.27 &                 -4.51 \\
GaussianCopulaCategorical      &                -7.24 &                 -4.51 \\
\textbf{\model (ours)}                 &                -3.50 &                 -3.54 \\
IdentitySynthesizer            &                -3.47 &                 -3.49 \\
IndependentSynthesizer         &                -3.47 &                 -3.49 \\
\bottomrule
\end{tabular}


==> tables/gridr.tex <==
\begin{tabular}{lrr}
\toprule
{} &  gridr/syn\_likelihood &  gridr/test\_likelihood \\
\midrule
MedganSynthesizer              &                 -7.37 &                -141.41 \\
VEEGANSynthesizer              &                -11.46 &                  -8.91 \\
CLBNSynthesizer                &                 -4.01 &                  -7.43 \\
PrivBNSynthesizer              &                 -4.07 &                  -7.12 \\
CTGAN                          &                 -8.31 &                  -5.05 \\
CTGANSynthesizer               &                 -8.32 &                  -5.03 \\
CopulaGAN                      &                 -8.16 &                  -5.01 \\
TableganSynthesizer            &                 -7.00 &                  -4.83 \\
UniformSynthesizer             &                 -7.22 &                  -4.57 \\
GaussianCopulaCategoricalFuzzy &                 -7.14 &                  -4.55 \\
GaussianCopulaOneHot           &                 -7.19 &                  -4.55 \\
GaussianCopulaCategorical      &                 -7.16 &                  -4.54 \\
IndependentSynthesizer         &                 -5.12 &                  -4.03 \\
\textbf{\model (ours)}                 &                 -3.89 &                  -3.71 \\
TVAESynthesizer                &                 -3.87 &                  -3.71 \\
IdentitySynthesizer            &                 -3.59 &                  -3.64 \\
\bottomrule
\end{tabular}


==> tables/insurance.tex <==
\begin{tabular}{lrr}
\toprule
{} &  insurance/syn\_likelihood &  insurance/test\_likelihood \\
\midrule
UniformSynthesizer             &                    -18.42 &                     -18.42 \\
VEEGANSynthesizer              &                    -18.33 &                     -18.11 \\
GaussianCopulaOneHot           &                    -17.84 &                     -17.91 \\
IndependentSynthesizer         &                    -18.38 &                     -17.57 \\
GaussianCopulaCategorical      &                    -17.84 &                     -16.58 \\
GaussianCopulaCategoricalFuzzy &                    -18.03 &                     -16.52 \\
MedganSynthesizer              &                    -13.88 &                     -15.08 \\
CTGAN                          &                    -17.03 &                     -14.97 \\
CopulaGAN                      &                    -16.96 &                     -14.96 \\
CTGANSynthesizer               &                    -16.60 &                     -14.84 \\
TableganSynthesizer            &                    -16.18 &                     -14.32 \\
TVAESynthesizer                &                    -14.30 &                     -14.24 \\
CLBNSynthesizer                &                    -15.17 &                     -13.92 \\
PrivBNSynthesizer              &                    -14.70 &                     -13.64 \\
\textbf{\model (ours)}                 &                    -13.21 &                     -13.11 \\
IdentitySynthesizer            &                    -12.85 &                     -12.96 \\
\bottomrule
\end{tabular}


==> tables/intrusion.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  intrusion/accuracy &  intrusion/macro\_f1 &  intrusion/micro\_f1 \\
\midrule
UniformSynthesizer             &                0.12 &                0.07 &                0.12 \\
VEEGANSynthesizer              &                0.51 &                0.18 &                0.51 \\
IndependentSynthesizer         &                0.72 &                0.20 &                0.72 \\
GaussianCopulaCategorical      &                0.79 &                0.18 &                0.79 \\
GaussianCopulaCategoricalFuzzy &                0.84 &                0.26 &                0.84 \\
MedganSynthesizer              &                0.87 &                0.27 &                0.87 \\
GaussianCopulaOneHot           &                0.90 &                0.33 &                0.90 \\
CLBNSynthesizer                &                0.94 &                0.39 &                0.94 \\
PrivBNSynthesizer              &                0.95 &                0.38 &                0.95 \\
TVAESynthesizer                &                0.97 &                0.43 &                0.97 \\
CTGANSynthesizer               &                0.98 &                0.51 &                0.98 \\
CopulaGAN                      &                0.98 &                0.52 &                0.98 \\
CTGAN                          &                0.98 &                0.54 &                0.98 \\
\textbf{\model (ours)}                 &                0.99 &                0.59 &                0.99 \\
IdentitySynthesizer            &                1.00 &                0.86 &                1.00 \\
\bottomrule
\end{tabular}


==> tables/news.tex <==
\begin{tabular}{lr}
\toprule
{} &       news/r2 \\
\midrule
VEEGANSynthesizer              & -319605180.25 \\
GaussianCopulaOneHot           &        -36.94 \\
GaussianCopulaCategoricalFuzzy &         -8.66 \\
CLBNSynthesizer                &         -6.47 \\
TableganSynthesizer            &         -5.82 \\
MedganSynthesizer              &         -5.60 \\
GaussianCopulaCategorical      &         -5.03 \\
UniformSynthesizer             &         -4.44 \\
CTGANSynthesizer               &         -0.51 \\
TVAESynthesizer                &         -0.24 \\
CTGAN                          &         -0.07 \\
IndependentSynthesizer         &         -0.06 \\
CopulaGAN                      &         -0.06 \\
\textbf{\model (ours)}                 &          0.11 \\
IdentitySynthesizer            &          0.13 \\
\bottomrule
\end{tabular}


==> tables/ring.tex <==
\begin{tabular}{lrr}
\toprule
{} &  ring/syn\_likelihood &  ring/test\_likelihood \\
\midrule
MedganSynthesizer              &                -2.78 &               -149.77 \\
CLBNSynthesizer                &                -1.77 &                -47.16 \\
VEEGANSynthesizer              &               -16.83 &                 -6.35 \\
CopulaGAN                      &                -6.21 &                 -2.80 \\
CTGANSynthesizer               &                -7.13 &                 -2.70 \\
CTGAN                          &                -6.59 &                 -2.67 \\
TableganSynthesizer            &                -4.74 &                 -2.53 \\
UniformSynthesizer             &                -5.34 &                 -2.50 \\
GaussianCopulaOneHot           &                -3.21 &                 -2.15 \\
GaussianCopulaCategoricalFuzzy &                -3.18 &                 -2.15 \\
GaussianCopulaCategorical      &                -3.20 &                 -2.15 \\
IndependentSynthesizer         &                -2.47 &                 -1.96 \\
TVAESynthesizer                &                -1.58 &                 -1.94 \\
\textbf{\model (ours)}                 &                -1.82 &                 -1.74 \\
IdentitySynthesizer            &                -1.71 &                 -1.70 \\
\bottomrule
\end{tabular}


==> tables/summary.tex <==
\begin{tabular}{llc}
\toprule
         &           & \model rank \\
Dataset Type & Dataset &            \\
\midrule
real & adult &          1 \\
         & census &          1 \\
         & covtype &          1 \\
         & credit &          3 \\
         & intrusion &          1 \\
         & news &          1 \\
synthetic & grid &          2 \\
         & gridr &          2 \\
         & ring &          1 \\
bayesian & alarm &          1 \\
         & asia &          2 \\
         & child &          1 \\
         & insurance &          1 \\
\bottomrule
\end{tabular}


==> tables/summary_compact.tex <==
\begin{tabular}{p{0.1\textwidth}p{0.24\textwidth}p{0.06\textwidth}}
\toprule
Dataset Type & Dataset & \model{} rank \\
\midrule
real & \emph{adult}, \emph{census}, \emph{covtype}, \emph{intrusion} and \emph{news} & 1 \\
 & \emph{credit} & 3 \\
\midrule
synthetic & \emph{ring} & 1 \\
 & \emph{grid} and \emph{gridr} & 2 \\
\midrule
bayesian & \emph{alarm}, \emph{child} and \emph{insurance} & 1 \\
 & \emph{asia} & 2 \\
\bottomrule
\end{tabular}

